Reconfigurable Intelligent Surface Enabled Spatial Multiplexing with Fully Convolutional Network

Reconfigurable intelligent surface (RIS) is an emerging technology for future wireless communication systems. In this work, we consider downlink spatial multiplexing enabled by the RIS for weighted sum-rate (WSR) maximization. In the literature, most solutions use alternating gradient-based optimization, which has moderate performance, high complexity, and limited scalability. We propose to apply a fully convolutional network (FCN) to solve this problem, which was originally designed for semantic segmentation of images. The rectangular shape of the RIS and the spatial correlation of channels with adjacent RIS antennas due to the short distance between them encourage us to apply it for the RIS configuration. We design a set of channel features that includes both cascaded channels via the RIS and the direct channel. In the base station (BS), the differentiable minimum mean squared error (MMSE) precoder is used for pretraining and the weighted minimum mean squared error (WMMSE) precoder is then applied for fine-tuning, which is nondifferentiable, more complex, but achieves a better performance. Evaluation results show that the proposed solution has higher performance and allows for a faster evaluation than the baselines. Hence it scales better to a large number of antennas, advancing the RIS one step closer to practical deployment.

==> coverletter.tex <==
Dear editor,

Please find attached our manuscript "Reconfigurable intelligent surface enabled spatial multiplexing with fully convolutional network", which we would like to submit for publication as an original research article in IEEE Transactions on Wireless Communications. Our main contribution is to apply a fully convolutional network (FCN) to the RIS configuration for spatial multiplexing. The FCN was invented for computer vision. To our best knowledge, it has not yet been applied to RIS signal processing. Evaluation results show that the proposed approach not only achieves higher weighted sum-rate than the state-of-the-art algorithm, but requires much less computation time, which allows for an easier deployment of real-time application.

This work has not been submitted elsewhere.
The corresponding author is Bile Peng (peng@ifn.ing.tu-bs.de).
We are looking forward to hearing from you.

Sincerely,

Bile Peng, Jan-Aike Termöhlen, Cong Sun, Danping He, Ke Guan, Tim Fingscheidt, Eduard Jorswieck


V2:

Dear editor,

Please find attached our manuscript "Reconfigurable intelligent surface enabled spatial multiplexing with fully convolutional network", which we would like to submit for publication as an original research article in IEEE Transactions on Signal Processing. Our main contribution is to apply a fully convolutional network (FCN) to the RIS configuration for spatial multiplexing. The FCN was invented for computer vision. To our best knowledge, it has not yet been applied to RIS signal processing. Evaluation results show that the proposed approach not only achieves higher weighted sum-rate than the state-of-the-art algorithm, but requires much less computation time, which allows for an easier deployment of real-time application.

This manuscript was rejected by IEEE Transactions on Wireless Communications (Paper-TW-Dec-21-1786). Before the submission to IEEE TSP, we thoroughly improved the manuscript by generalizing the method to an arbitrary number of users, considering imperfect channel state information and discrete phase shifts. Besides, we have improved the presentation such that telecommunication experts who are not very familiar with machine learning can understand the manuscript more easily. Details of the revision can be found in the response letter.

The corresponding author is Bile Peng (peng@ifn.ing.tu-bs.de).

We are looking forward to hearing from you.

Sincerely,

Bile Peng, Ke Guan, Danping he, Jan-Aike Termöhlen, Cong Sun, Tim Fingscheidt, Eduard Jorswieck
